FedCert: Federated Accuracy Certification

Federated Learning (FL) has emerged as a powerful paradigm for training machine learning models in a decentralized manner, preserving data privacy by keeping local data on clients. However, evaluating the robustness of these models against data perturbations on clients remains a significant challenge. Previous studies have assessed the effectiveness of models in centralized training based on certified accuracy, which guarantees that a certain percentage of the model's predictions will remain correct even if the input data is perturbed. However, the challenge of extending these evaluations to FL remains unresolved due to the unknown client's local data. To tackle this challenge, this study proposed a method named FedCert to take the first step toward evaluating the robustness of FL systems. The proposed method is designed to approximate the certified accuracy of a global model based on the certified accuracy and class distribution of each client. Additionally, considering the Non-Independent and Identically Distributed (Non-IID) nature of data in real-world scenarios, we introduce the client grouping algorithm to ensure reliable certified accuracy during the aggregation step of the approximation algorithm. Through theoretical analysis, we demonstrate the effectiveness of FedCert in assessing the robustness and reliability of FL systems. Moreover, experimental results on the CIFAR-10 and CIFAR-100 datasets under various scenarios show that FedCert consistently reduces the estimation error compared to baseline methods. This study offers a solution for evaluating the robustness of FL systems and lays the groundwork for future research to enhance the dependability of decentralized learning. The source code is available at https://github.com/thanhhff/FedCert/.

==> Chapters/3-1backup.tex <==
\noindent \textbf{Problem Definition.} 
Consider a Federated Learning (FL) system with \( N \) clients, where each client \( i \) has a local dataset \( D_i \). This study focuses on the classification problem, specifically in scenarios where the datasets \( D_i \) (for \( i = \{1, \ldots, N\} \)) contain the same set of classes. Let \( \theta \) represent the global model obtained after the federated learning process. Our goal is to certify the accuracy of \( \theta \) when it is deployed in practice. However, since the server does not have access to a test dataset, conventional accuracy certification methods cannot be applied. To this end, we assume the server has knowledge of the class distribution in practice, denoted as \( p(S) \), where \( S \) represents the data in practice (this assumption is reasonable, as class distributions often follow a uniform distribution). Given \( p(S) \), our task is to estimate the certified accuracy of \( \theta \) with respect to \( S \) within a specified test radius \( r \).\\


% , and \( S \) be the 
% Let \( S \) represent a test set that includes all the classes, with an IID distribution across those classes.
% The global model obtained after the communication process is denoted by \( \theta \). 
% Estimating the certified accuracy of the FL system involves evaluating the certified accuracy of \( \theta \) on a test set \( S \) at a specified radius \( r \).
% Notably, the server has no access to samples from \( S \). 
% The distribution of \( S \) may either correspond with the clients' distributions (i.e., when all clients have IID data) or differ from them.


% After federated training, we obtain the global model weights $\theta$. 
% Assuming we want to evaluate the certified accuracy on a test dataset $S$ with label proportion $p(S)$ using the model weights $\theta$ under the test radius $r$. 
% However, we cannot access to the raw data on $S$ due to privacy constraints. 
% The problem is to estimate the certified accuracy $c(\theta, S, r)$ using $p(S)$ through the test datasets of the clients.
% \\

\noindent \textbf{Motivation.} 
% In this context, we use the term ``test dataset'' $S$ in FL similarly to the test dataset in centralized learning, where both training and testing sets are provided. However, in FL, due to privacy concerns, consolidating raw data to create a sufficiently large test dataset is infeasible.
% The label proportion of a dataset $E$ in a classification task, which might be predefined by domain-specific knowledge, is denoted as $P(E)$. We approximate the certified accuracy on $S$ based on its label proportion $p(S)$.
% In this context, we use the term ``test dataset'' $S$ in FL similarly to its use in centralized learning, where both training and testing sets are provided. 
% However, due to privacy concerns in FL, consolidating raw data to create a sufficiently large test dataset is infeasible. 
% The label distribution of a dataset $E$ in a classification task, which might be predefined by domain-specific knowledge, is denoted as $P(E)$. We approximate the certified accuracy on $S$ based on its label distribution $p(S)$.
% In traditional machine learning, the model obtained after training is evaluated on a prepared test dataset depending on the evaluation purpose. However, in the FL environments, we don't have a test dataset to evaluate the performance of the global model because of the difficulty of collecting raw data. In this research, we defined the term ``test dataset'' $S$ as a wanted evaluation dataset. Although we cannot collect raw data to evaluate directly on $S$, label distribution $p(S)$ can be predefined based on the evaluation purpose. We compute the certified accuracy of this ``test dataset'' $S$ with this predefined label distribution. 


% In FL settings, let $N$ denote the number of clients, and $D_i$ represent the local test dataset of client $i$. The union of all local test datasets is $D = \{D_1 \cup D_2 \cup \ldots \cup D_N\}$. $D$ can be either IID or non-IID with respect to $S$, where the set of classes in $S$ and $D$ is identical.
% After the global model has converged, we obtain the model parameters $\theta$. The certified accuracy of client $i$, evaluated using the model $\theta$ on the local test dataset $D_i$ under a test radius $r$, is denoted as $c(\theta, D_i, r)$. 

As previously mentioned, directly certifying the theta model on the dataset \( S \) is not feasible because, in a federated learning context, the server typically does not have access to the data. To this end, our main approach involves allowing each client to certify the accuracy of $\theta$ on its local dataset. These local certified accuracy are then combined linearly by the server produce the estimated certified accuracy of $\theta$ on \( S \).
Specifically, let \( c(\theta, D_i, r) \) represents the accuracy of $\theta$ certified by client \( i \) on its dataset \( D_i \) within radius \( r \), the certified accuracy of $\theta$ with respect to \( S \) can then be estimated using the following formula:
\begin{equation}
    c(\theta, S, r) \approx \sum_{i=1}^N{\alpha_i}c(\theta,D_i, r).
\end{equation}
Our problem deduce to determine $\alpha_i$ ($i = 1, ..., n$) to satisfy the following objective function: 
\begin{equation}
    \underset{\{\alpha_i\}_{i=1}^{N}}{argmin}{\left|c(\theta, S, r) - \sum_{i=1}^{N}\alpha_ic(\theta, D_i, r) \right| }.
\end{equation}


\begin{align*}
    \min \left\| c(\theta,S, r) - \mathcal{L}(c(\theta,D_1, r), c(\theta,D_2, r), \dots, c(\theta,D_N, r)) \right\|.
\end{align*}

% The key challenge here is determining the appropriate weights \( \alpha_i \).

% To address the problem, we propose an algorithm that estimates the certified accuracy on dataset $S$ by aggregating the certified accuracy from individual clients. The formulation of our solution as an optimization problem is given by:

% We toward designing $\mathcal{L}$ as a linear combination of the clients’ certified accuracies.
% Further analysis of the certified accuracy of a dataset, which is the union of other datasets, supports our observations as detailed in Observation 2. Additionally, we provide a bound for our proposal in Proposition.

% Let:
% \begin{itemize}
%     \item $N$: the number of clients.
%     \item $D_i$: the local test dataset of client $i$, for $i = 1, 2, \ldots, N$.
%     \item $r$: the test radius.
%     \item $c(\theta,D_i, r)$: the certified accuracy of client $i$'s data $D_i$ for radius $r$, as defined in \cite{cohen2019certified} with classifier $f$.
%     \item $p(S)$: the desired global data distribution.
%     \item $p_{i \in N}(S)$: the percentage of label $i$ in the overall data according to the distribution $p(S)$.
% \end{itemize}
% We want to evaluate the certified accuracy of $p(S)$ under a test radius $r$ with model $f$. In centralized learning, where testing data is provided, we compute certified accuracy on the test set. However, in the scenario of federated learning, we cannot create a centralized dataset to test because of privacy and the impossibility of collecting data in nature. Therefore, we propose a method to estimate the certified accuracy of $p(S)$ over the certified accuracy of clients.

% \noindent \textbf{Problem Formulation}
% Given:
% \begin{itemize}
%     \item Local test datasets $D_i$ for each client $i$.
%     \item Certified accuracy $c(\theta,D_i, r)$ for each client $i$ and radius $r$.
%     \item Desired global data distribution $p(S)$.
% \end{itemize}
% The server needs to aggregate the certified accuracy from each client $i$ to approximate the certified accuracy as if it were evaluated directly on $p(S)$.
% \[
% c_{agg}(r) = s(c(\theta,D_1, r), c(\theta,D_2, r), \ldots, c(\theta,D_N, r)),
% \]
% Formally, let $c(\theta,p(S), r)$ represent the certified accuracy for the global distribution $p(S)$ at radius $r$. Where $s$ is the aggregation function that combines the certified accuracy of individual clients to approximate the certified accuracy for the desired global distribution. The goal is to design the aggregation function $s$ such that:
% \[
% |c_{agg}(r) - c(\theta,p(S), r)| \text{ is minimized}.
% \]
% % We begin with the theoretical analysis of the current limitations and our motivation in Section~\ref{subsec:theoretical_analysis}. Then, we provide a detailed practical algorithm in Section~\ref{subsec:practical_algorithm}.
% We toward designing $s$ as a linear combination of certified accuracy of clients by computing the weight for each client. In Section ~\ref{subsec:theoretical_analysis}, we analyze how data distribution skewness impacts the approximated certified accuracy when combining clients' certified accuracies linearly. Then, we provide a detailed practical algorithm in Section ~\ref{subsec:practical_algorithm}.

\subsection{Theoretical Analysis}
\label{subsec:theoretical_analysis}
% \subsubsection{Theorem 1.} Aggregation of clients' certified accuracy via weighted-sum aggregation based on clients' data volume. \\

\noindent \textbf{Observation 1.}   Suppose $\mathcal{T} = \{\mathcal{T}_1 \cup \mathcal{T}_2 \cup \ldots \cup \mathcal{T}_N\}$ where $\mathcal{T}_i$ is an individual test dataset. Let $n_i$ is the volume of $\mathcal{T}_i$, and $n$ is the volume of $\mathcal{T}$. The certified accuracy of $\mathcal{T}$ is equal to the linear combination of the certified accuracy of $\mathcal{T}_i$ with coefficients $n_i / n_\mathcal{T}$ under the same test radius $r$ and classifier~$\theta$.\\
\textbf{Proof.} Since $\mathcal{T} = \{\mathcal{T}_1 \cup \mathcal{T}_2 \cup \ldots \cup \mathcal{T}_N\}$, then $n^{robust}_{\mathcal{T}}(r) = \sum_{i=1}^{K} n^{robust}_{\mathcal{T}_i}(r)$. By definition, the certified accuracy on $\mathcal{T}$ can be calculated as follows:
\begin{equation*}
    % c(\theta,\mathcal{T}, r) = \frac{n^{robust}_{\mathcal{T}_i(r)}{n_D} = \frac{\sum_{i=1}^{K} n^{robust}_{\mathcal{T}_i}(r)}{n_{\mathcal{T}}}
        % = \sum_{i=1}^{K} \left( \frac{n_{\mathcal{T}_i}}{n_{\mathcal{T}}} c(\theta,\mathcal{T}_i, r) \right).
        c(\theta,\mathcal{T}, r) = \frac{n^{robust}_{\mathcal{T}}}{n_\mathcal{T}} = \frac{\sum_{i=1}^{N}n^{robust}_{\mathcal{T}_i}(r)}{n_{\mathcal{T}}}
        = \sum_{i=1}^{N}  \frac{n_{\mathcal{T}_i}}{n_{\mathcal{T}}} c(\theta,\mathcal{T}_i, r).
\end{equation*}
The observation presents a straightforward method to compute the certified accuracy across all data without merging or centralizing the clients' test datasets. This approach evaluates the certified accuracy of the combined client test data by aggregating the certified accuracies of individual clients, weighted by the volume of each client's test dataset. This method allows for the assessment of the aggregated test dataset's certified accuracy while preserving data privacy, provided that $p(S)$ closely matches the label distribution of the clients' combined test dataset. However, this approach may be inadequate if the label distribution of the clients' union test dataset does not represent the target distribution.\\
\textbf{Observation 2.} The relation between the expected certified accuracy of clients' label distribution \( p(D) \) and the desired label distribution \( p(S) \).
\begin{align}
\nonumber
    &\text{If } p(S) = \sum_{i=1}^{N}{w_i p(D_i)}, \quad \sum_{i=1}^{N}{w_i} = 1, \quad 0 \leq w_i \leq 1; \\
    &\text{then,  } \mathbf{E}_{S \sim p(S)}[c(\theta,S, r)] = \sum_{i=1}^{N}{w_i \mathbf{E}_{D_i \sim p(D_i)}\left[c(\theta,D_i, r)\right]}. \nonumber
\end{align}
\textbf{Proof.} Let $S^i$ be the set containing samples belonging to class $i$ of $S$ and $a_i(S)$ be the proportion of $S^i$ in $S$. From Observation 1, we have: $c(S) = a_i(S)\sum c(\theta, S^i, r)$, therefore, we have:
\begin{equation*}
    \mathbf{E}_{S \sim p(S)}[c(\theta,S, r)] = a_j(S)\sum_{j} \mathbf{E}_{S^j \sim p(S^j)}[c(\theta,S^j, r)]
\end{equation*}
\begin{equation*}
    \mathbf{E}_{D_i \sim p(D_i)}[c(\theta,D_i, r)] = a_j(D_i)\sum_{j} \mathbf{E}_{D_i^j \sim p(D_i^j)}[c(\theta,D_i^j, r)]
\end{equation*}
We have $p(S) = \sum_{i=1}^{N}{w_i p(D_i)}$, that mean:
\begin{equation*}
    a_j(S) = \sum_{i} w_i a_j(D_i)
\end{equation*}
Also,
\begin{equation*}
 \mathbf{E}_{S^j \sim p(S^j)}[c(\theta,S^j, r)] = \mathbf{E}_{D_i^j \sim p(D_i^j)}[c(\theta,D_i^j, r)]    
\end{equation*}
because $p(S^j) = p(D^j_i)$ . Then:
\begin{equation*}
    a_j(S)\mathbf{E}_{S^j \sim p(S^j)}[c(\theta,S^j, r)] = \sum_{i} w_i a^j_i \mathbf{E}_{D_i^j \sim p(D_i^j)}[c(\theta,D_i^j, r)]
\end{equation*}
Add the sum of both sides, we prove Observation 2.

Observation 2 provides a theoretical foundation for aggregating clients' certified accuracy using weighted-sum aggregation based on label distribution.
If the weights \( w_i \) can be determined, the certified accuracy can be easily computed. 
However, the condition \( p(S) = \sum_{i=1}^{N}{w_i p(D_i)} \) poses challenges for integration into FL, making the application of observation 2 difficult. 
To address this problem, instead of satisfying the condition, we aim to minimize the distance $ ||p(S) - \sum_{i=1}^{N}{w_i p(D_i)} ||$. 
This approach is equivalent to finding the aggregated weights by solving the following optimization problem:
\begin{align*}
w^* = \operatorname{argmin} \; \left\|p(S) - \sum_{i=1}^{N}{w_i p(D_i)} \right\|, \\ 
\sum_{i=1}^{N}{w_i} = 1, \quad 0 \leq w_i \leq 1.
\end{align*}
\textbf{Proposition.} Let \(\delta = \left\| p(S) - \sum_{i=1}^N w^*_i p(D_i) \right\|\), then we have:
\begin{equation}
\nonumber
    \left\| c(\theta,S, r) - \sum_{i=1}^N w^*_i c(\theta,D_i, r) \right\| \leq \delta Q,
\end{equation}
with $Q$ is independent of $w$.

\noindent \textbf{Proof. }
For convenience, we denote \(L_i(r)\) as the certified accuracy of class \(i\) under the test radius \(r\), \(p_i\) as the probability of class \(i\) under \(p(S)\), and \(p'_i\) as the probability of class \(i\) under the approximation distribution. We have: \(p(S') = \sum_{i=1}^{K} w_i p(D_i) = [p'_1, \ldots, p'_N]\).
Then, by Theorem 2, we have:
\begin{equation}
\nonumber
    \begin{cases}
        c(\theta,S, r) &= \sum_{i=1}^{N} p_i L_i(r), \\
        c'(\theta, S, r) &= \sum_{i=1}^{N} p'_{i} L_i(r).
    \end{cases}
\end{equation}
The bound of the gap between the approximation and the ground truth can be represented by the following function:
\[ H = \left \|c(\theta,S, r) - c'(\theta, S, r) \right \|. \]
This problem can be viewed as a convex optimization problem as follows:
\begin{align*}
    &\max \left \|\sum_{i=1}^{N}(p_i - p'_i)L_i(r) \right \|, \\ &\text{subject to:}
    \begin{cases}
        \sum_{i=1}^{N}(p_i - p'_i)^2 &\leq \delta^2, \\
        \sum_{i=1}^{N}(p_i - 1) &= 0.
    \end{cases}
\end{align*}
To solve this problem, we address the following subproblems:
\begin{align*}
\begin{cases}
    \min f(p') &= \sum_{i=1}^{N}(p'_i - p_i)L_i(r), \\
    \max g(p') &= \sum_{i=1}^{N}(p'_i - p_i)L_i(r).
\end{cases}
\end{align*}
We first solve the optimization problem \( f(p') \) by applying the Karush Kuhn Tucker (KKT) conditions. Since \( f(p') \) is an affine function, the solution of the KKT conditions is the global solution:
% \begin{align}
%     & \sum_{i=1}^{N}(p_i - p_i')^2 \leq \delta^2, \nonumber \\
%     & \sum_{i=1}^{N}p_i - 1 = 0, \nonumber \\
%     & a \left[ \sum_{i=1}^{N}(p_i - p_i')^2 - \delta^2 \right] = 0, \nonumber \\
%     & L_i(r) - 2a(p'_i - p_i) + b = 0 \quad \text{for } i = 1, \ldots, N. \label{2.4}
% \end{align}
% 
\begin{align}
    \left\{
    \begin{array}{ll}
        \sum_{i=1}^{N}(p_i - p_i')^2 \leq \delta^2, \\[5pt]
        \sum_{i=1}^{N}p_i - 1 = 0, \\[5pt]
        a \left[ \sum_{i=1}^{N}(p_i - p_i')^2 - \delta^2 \right] = 0, \\[5pt]
        L_i(r) - 2a(p'_i - p_i) + b = 0 \quad \text{for } i = \{1, \dots, N\}.
    \end{array}
    \right.
    \label{2.4}
\end{align}
To solve this, we first sum all the equations in Eq.~\ref{2.4}:
\begin{align*}
    \sum_{i=1}^{N}L_i(r) + Nb = 0   \quad \Leftrightarrow \quad b = -\frac{\sum_{i=1}^{N}L_i(r)}{N}.
\end{align*}
% 
We denote \(\bar{L} = \frac{\sum_{i=1}^{N}L_i(r)}{N}\). Then, substituting the value of \(b\) in each equation in Eq.~\ref{2.4}:
\begin{align*}
    L_i(r) - 2a(p'_i - p_i) - \bar{L} = 0 \quad \Leftrightarrow \quad 2a(p'_i - p_i) = L_i(r) - \bar{L}.
\end{align*}
% 
Since \(a \neq 0\), we have:
\begin{align*}
    \begin{cases}
        p'_i - p_i &= \frac{L_i(r) - \bar{L}}{2a}, \\
        \sum_{i=1}^{N}(p'_i - p_i)^2 &= \delta^2.
    \end{cases}
\end{align*}
% 

Solving this system, we achieve the final solution:
\begin{align*}
    \begin{cases}
        b &= -\bar{L}, \\
        4a^2 &= \frac{\sum_{i=1}^{N}(L_i(r) - \bar{L})^2}{\delta^2}, \\
        p'_i - p_i &= \frac{L_i(r) - \bar{L}}{2a}.
    \end{cases}
\end{align*}
As shown above, the solution of the KKT equations is the global solution of the optimization problem. 
Applying this to \( f(p') \), we have:
\begin{align*}
    \min f(p') &= \sum_{i=1}^{N} \frac{(L_i(r) - \bar{L})L_i(r)}{2a} \\
               &= -\delta \frac{\sum_{i=1}^{N}(L_i(r) - \bar{L})L_i(r)}{\sqrt{\sum_{i=1}^{N}(L_i(r) - \bar{L})^2}}.
               % &= -\delta B.
\end{align*}
We have:
\begin{align*}
    \sum_{i=1}^{N}(L_i(r) - \bar{L})^2 
    &= \sum_{i=1}^{N}L_i(r)^2 -  2\bar{L}\sum_{i=1}^{N}L_i(r) + \bar{L}^2  \\
    &= \sum_{i=1}^{N}L_i(r)^2 - \bar{L}\left[ 2\sum_{i=1}^{N}L_i(r) - \sum_{i=1}^{N}{\bar{L}} \right] \\
    &= \sum_{i=1}^{N}L_i(r)^2 - \bar{L}\sum_{i=1}^{N}L_i(r) \\
    &= \sum_{i=1}^{N}(L_i(r) - \bar{L})L_i(r).
\end{align*}
% 
Therefore:
\begin{align*}
    \min f(p') &= -\delta \sqrt{\sum_{i=1}^{N}(L_i(r) - \bar{L})^2}.
\end{align*}
% 
Similarly, we can prove that:
\begin{align*}
    \max g(p') = \delta \sqrt{\sum_{i=1}^{N}(L_i(r) - \bar{L})^2}.
\end{align*}
% 
Thus, we have the bound on the gap between the approximated result and the ground truth:
\begin{equation}
    \label{bound}
    H \leq \delta \sqrt{\sum_{i=1}^{N}(L_i(r) - \bar{L})^2} = \delta Q.
\end{equation}
Eq.~\ref{bound} demonstrates two key points:
\begin{itemize}
\item As $\delta$ becomes smaller, the optimization result also becomes smaller. This indicates that the closer the approximate distribution is to the target distribution, the more accurate the result.
\item When the certified accuracy of each class becomes more similar to each other, the bound approaches zero.
\end{itemize}



==> Chapters/5-Relatedwork.tex <==
% One of the challenges in machine learning is adversarial attacks, which aim to fool a learned model into making mistakes by adding small, carefully crafted perturbations to the input data. 
% These perturbations are often negligible to human perception but significantly affect the network's outcomes. 
% To address this issue, adversarial defense techniques have been developed to enhance machine learning robustness. 
% There are two common approaches: Empirical Defense and Certified Defense \cite{nandy2022bridging}. The former demonstrates empirical robustness against adversarial attacks without providing any certification guarantee, usually by optimizing the task-specific loss function given perturbations $\sigma$. Let $\sigma \in \Delta$ with $\Delta = \{\epsilon: ||\epsilon|| \leq \sigma\}$, the general objective function to enhance robustness can be described as follows:
% \begin{equation}
% \nonumber
%     \min_{\theta} \mathbb{E}_{(x,y)}[\max_{\epsilon\in\Delta}L(f_{\theta}(x+\sigma),y)],
% \end{equation}
% where $\theta$ denotes the model parameters and $L(.)$ is the task-specific loss. Certified robustness, on the other hand, refers to a provable assurance that a machine learning model will perform consistently well within a predetermined range of noises and perturbations. A classifier, typically a neural network, is said to be certifiably robust if for any input $x$, there is a guarantee that the classifier’s outcome is constant within some set around $x$, typically an $l_2$ or $l_{\infty}$ ball. Among various methods in this field, randomized smoothing is a promising certification technique that can be scaled to large networks and higher-dimensional datasets.

Research on the robustness of FL primarily examines the effects of adversarial attacks on the FL system and devises algorithms to address them. 
One approach is Federated Adversarial Training (FAT)~\cite{li2023federated}, which deploys an adversarial training scheme on local clients for the conventional FL algorithm FedAvg~\cite{mcmahan2017communication}.
Moreover, building on the centralized methods from~\cite{salman2019provably} and~\cite{liu2020primer}, Chen et al.~\cite{chen2021certifiablyrobust} integrated randomized smoothing into FL and applied adversarial training to update the local model. This approach uses a volume-based aggregated global model similar to FedAvg to evaluate the robustness of the FL system.
Additionally, Alfarra et al.~\cite{alfarra2022certified} investigated the benefits of FL on certified robustness using diverse perturbation methods, including Gaussian noise, rotation, and pixel perturbations locally. 
Several studies have also theoretically analyzed the robustness of FL under noise. 
Yin et al.\cite{yin2018byzantine} developed a robust distributed optimization algorithm against arbitrary adversarial behavior and focused on achieving optimal statistical performance. 
Reisizadeh et al.~\cite{reisizadeh2020robust} introduced a robust FL algorithm by considering the structured affine distribution shift in users' data.

% One of challenges in machine learning is adversarial attack which aims to fool a learned model to make mistakes via adding small, carefully crafted perturbations to the input data. 
% These perturbations are often negligible to human perception but strongly affect networks' outcomes. 
% To deal with this problem, adversarial defense as a set of techniques for machine learning adversarial-robustness enhancement is designed. 
% There are two common approaches namely Empirical defense and Certified defense\cite{nandy2022bridging}. 
% The former demonstrate empirical robustness against adversarial attacks without providing any certification guaranteed, usually by optimizing the task-specific loss function given perturbations $\sigma$. 
% Let $\sigma\in\Delta$ with $\Delta = \{\epsilon: ||\epsilon|| \leq \sigma\}$, the general objective function to enhance robustness can be described as follows:
% \begin{equation}
% \nonumber
%     \min_{\theta} \mathbb{E}_{(x,y)}[\max_{\epsilon\in\Delta}L(f_{\theta}(x+\sigma),y)]
% \end{equation}
% where $\theta$ denotes the model parameters and $L(.)$ is the task-specific loss. Certified robustness, on the other hand, refers to a provable assurance that a machine learning model will perform consistently well within a predetermined range of noises and perturbations. A classifier, typically as a neural network, is said to be certifiably robust if for any input $x$,  a guarantee that the classifier’s outcome is constant within some set around
% $x$, typically an $l_2$ or $l_{\infty}$ ball can be easily obtained. Among various methods in this field, randomized smoothing is a promising certification technique that can be scaled to large networks and higher-dimensional datasets. 

% Research on the robustness of FL primarily examines the effects of adversarial attacks on the FL system and devises algorithms to address them. Regarding to recent developed methods, Federated Adversarial Training (FAT) \cite{li2023federated} deployed the adversarial training scheme on local clients for the conventional FL algorithm FedAvg \cite{mcmahan2017communication}. 
% Integrating randomized smoothing to FL, \cite{chen2021certifiablyrobust} apply adversarial training to the local model update based on the centralized ones introduced in \cite{salman2019provably}, \cite{liu2020primer} with volume-based aggregated global model as FedAvg. 
% Also, by using diverse perturbation methods including Gaussian noise, rotation, and pixel perturbations locally, \cite{alfarra2022certified} investigated the benefits of FL on certified robustness. 
% Besides that, there were several works that theoretically analyzed the robustness of FL under noise. \cite{yin2018byzantine} developed a distributed optimization algorithm that were provably robust against arbitrary adversarial behavior and mainly focused on achieving optimal statistical performance. 
% \cite{reisizadeh2020robust} introduced a robust FL algorithm via consideration of the structured affine distribution shift in users' data.

